MUSIC-lite: Efficient MUSIC using Approximate Computing: An OFDM Radar Case Study

Multiple Signal Classification (MUSIC) is a widely used Direction of Arrival (DoA)/Angle of Arrival (AoA) estimation algorithm applied to various application domains such as autonomous driving, medical imaging, and astronomy. However, MUSIC is computationally expensive and challenging to implement in low-power hardware, requiring exploration of trade-offs between accuracy, cost, and power. We present MUSIC-lite, which exploits approximate computing to generate a design space exploring accuracy-area-power trade-offs. This is specifically applied to the computationally intensive singular value decomposition (SVD) component of the MUSIC algorithm in an orthogonal frequency-division multiplexing (OFDM) radar use case. MUSIC-lite incorporates approximate adders into the iterative CORDIC algorithm that is used for hardware implementation of MUSIC, generating interesting accuracy-area-power trade-offs. Our experiments demonstrate MUSIC-lite's ability to save an average of 17.25% on-chip area and 19.4% power with a minimal 0.14% error for efficient MUSIC implementations.

==> Text/background.tex <==

\section{Developmental Ideas}
    \label{sec:background}
     In this section, we discuss the preliminaries behind our idea and design. The popular adder proposed in literature is the ripple-carry adder~\cite{cla}. However, the ripple-carry adder suffers from substantial delays as it has to wait for the carry-bit to propagate from the LSB point to the MSB. There can be some potential approximations that can be achieved via reducing the carry chain~\cite{cesa} or using a modified carry select scheme~\cite{hu} to name a few. Towards reducing the dependencies on the previous bits, we introduce two units namely the Carry Judge Unit (CJU) and the Exact Carry Unit (ECU) as shown in Figure~\ref{fig:carry_estimate} which we shall now discuss. %In this section we discuss about the several proposed sub-blocks such as CJU (Carry Judge Unit) and ECU (Exact Carry Unit) from our proposed design as shown in Figure~\ref{fig:carry_estimate}. 
     
     The basic architecture of ACLA as shown in Figure~\ref{fig:carry_estimate} adds two $n$-bit input binary numbers by dividing them into $n/k$ blocks where $k$ is the size of each block. Each $n/k$ block is fed a divided n-bit binary number as input, each part having k bits. Each block of the adder consists of 3 units, namely, Exact Carry Unit (ECU), Carry Judge Unit (CJU) and Sub Adder with the addition of one OR gate. Since, our proposed adder is an approximate parallel adder. Each of its $n/k$ block are not dependent on its previous blocks for calculation of $C_{out}$. Only $C_{out}$ from the previous block is used as $C_{in}$ for the calculation of block sum.   
    \begin{figure*}[tb]
        \begin{center}
            \includegraphics[width=0.88\textwidth]{Text/images/adder4.png}
            \caption{Cascaded blocks of proposed adder ACLA}
            \label{fig:carry_estimate}
          
        \end{center}
    \end{figure*}        
    
    As the name suggests, ECU generates $C_{ECU}$ which is always exact and correct. Whenever $C_{ECU}$ $=$ $1$ then our $C_{out}$ for that block is correct but same could not be said for the case $C_{ECU}$ $=$ $0$. The CJU (Carry Judge Unit) predicts $C_{CJU}$ for its respective block which is then fed into an OR gate along with $C_{ECU}$. The overall equation for the $C_{out}$ can be written as shown in equation~\ref{EQ1}. Where the summation shows that the output generated by two units ECU and CJU are independent of each other. %We will see how in our further discussions.  
    
    \begin{equation}
        C_{out} = C_{ECU} + C_{CJU}
        \label{EQ1}
    \end{equation}
    
\subsection{Exact Carry Unit (ECU)}
The Exact Carry Unit (ECU) shown in Figure~\ref{fig:carry_estimate} uses only the most significant upper 3 bits of the given block size of $k$ bits. After thorough experimentation, it was decided to take 3 bits under consideration as upper bits have more chances of deciding the $C_{out}$ for that block as upper bits are much nearer to next block. As well as it resulted in optimum balance between computation time and hardware consumption. For example, most significant bit has a probability of 25\% (1-1 configuration, i.e., our MSBs are 1, and 1) to make $C_{out}$ = 1. While second most significant bits have a probability of 12.5\% (1-1 configuration for second most significant bit and 1-0 or 0-1 configuration for most significant bit) to make $C_{out} = 1$ by carry generated by it. ECU in turn uses the principle of the Carry-Lookahead Adder~\cite{cla} to compute $C_{ECU}$ as CLA has a low delay for transmitting the carry. 
\begin{equation}
    P_i = A_{i}\oplus B{i}
    \label{EQ2}
\end{equation}
\begin{equation}
    G_i = A_{i}.B_{i}
    \label{EQ3}
\end{equation}
So, using equation~\ref{EQ2} and \ref{EQ3} we can calculate $C_{ECU}$ for the given block.
\begin{equation}
    C_{ECU} = G_{0} + P_{0}.G_{1} + P_{0}.P_{1}.G_{2}
    \label{EQ4}
\end{equation}
%\begin{figure*}[h!]
    
 %       \includegraphics[width=0.45\textwidth]{Text/images/ecu(1).png}
  %      \caption{Gate level diagram for $C_{ECU}$}
   %     \label{fig:Cecu}
 
%\end{figure*}
Looking at equation~\ref{EQ4}, we can clearly see that if $C_{ECU} = 1$, then we can safely conclude that $C_{out}$ will be equal to $1$ and it will be correct since, in most cases of addition, $C_{out}$ can be calculated or predicted using most significant upper bits of the given block. We can even increase or decrease the accuracy of the adder by increasing or decreasing the number of most significant upper bits used for calculating $C_{ECU}$.

The probability of error is contingent upon the carry which is generated only by bits less significant than the upper 3 bits and is propagated by all the bits at more significant positions. Consider a block of size 8 and suppose carry is generated only by $A_5$ and $B_5$ digit of $i^{th}$ block. So, if this carry is propagated by the remaining more significant digits of the block, then a window for error occurs. To reduce the probability of such errors, we propose one more unit called the CJU. 

\subsection{Carry Judge Unit (CJU)}
Carry Judge Unit (CJU) estimates or predicts if the carry is generated by the bits which are less significant than the upper 3 bits. Suppose the block size is $k = 8$, then ECU will be responsible for evaluating if the carry is generated by the most significant upper 3 bits of the block, while CJU will be responsible for evaluating if the carry is generated by rest of the 5 lesser significant bits. Hence, output of two units are independent of each other.

In a typical Carry-Lookahead Adder, carry generation term as shown in equation~\ref{EQ2} is multiplied by carry propagation terms as shown in equation~\ref{EQ3} of bits more significant than it. This leads to higher power consumption, and delay in calculations. To reduce such overheads we propose following designs in the CJU :

    \begin{itemize}
%        \item Instead of multiplying each carry generation term (equation~\ref{EQ3}) with the more significant carry propagation terms (equation~\ref{EQ2}), we multiply the carry generation term (equation~\ref{EQ3}) of bits less significant than the upper 3 bits by carry propagation term (equation~\ref{EQ2}) of most significant upper 2 bits of the block as upper two bits play final deciding role in transmission of carry to the next block.
\item Instead of multiplying each carry generation term (equation~\ref{EQ3}) with the more significant carry propagation terms (equation~\ref{EQ2}), we multiply the carry generation term of bits less significant than the upper 3 bits by carry propagation term of most significant upper 2 bits of the block. The upper two bits play final deciding role in transmission of carry to the next block. This leads to reduction in area consumption and computation time.  
        \item  An Error Correction Term (ECT) as shown in equation~\ref{EQ5} will also be multiplied along with carry generation term which checks if $3^{rd}$ most significant bit of the block is propagating the carry generated or not.
    \end{itemize}
%instead of multiplying each carry generation term equation~\ref{EQ3} with all more significant carry propagation terms equation~\ref{EQ2} we multiply carry generation term equation~\ref{EQ3} of digits less significant than upper 3 bits only by carry propagation term equation~\ref{EQ2} of most significant upper 2 bits of the block and an Error Correction Term(ECT) equation~\ref{EQ5} which checks if $3^{rd}$ most significant bit of the block is propagating the carry generated or not.
    \begin{equation}
        \label{EQ5}
        ECT = A_2 | B_2 
    \end{equation}
    
    \begin{algorithm}
%        \begin{minipage}{0.9\linewidth}
            \caption{$C_{CJU}$ Calculation Algorithm}
            \label{alg:Ccju}
            \begin{algorithmic}[1]
                \STATE Initialize $factor$
                \STATE $P_0 = A_0 \oplus B_0$
                \STATE $P_1 = A_1 \oplus B_1$
                \STATE $ECT = A_2 | B_2$
                \FOR {$i = k - 1 \rightarrow 3$}
                \STATE $factor = factor + A_i . B_i$ 
                \ENDFOR
                \STATE $C_{CJU} = P_0 . P_1 . P_2 . ECT .factor$ \label{line:8}
            \end{algorithmic}
 %       \end{minipage}
    \end{algorithm}

   \begin{figure*}[tb]
        \begin{center}
            \mbox{ 
          %  \hspace{-1.0ex}
            \subfigure[Error Rate]
                {
                \label{fig:er}
                \includegraphics[width=0.4\textwidth]{Images/er.pdf}
                }
            
            \subfigure[NED]
                {
                \label{fig:ned}
                \includegraphics[width=0.4\textwidth]{Images/ned.pdf}
                }
           
            }
            \caption{Error Statistics}
            %\vspace{-3.0ex}
            \label{fig:error-parameters} 
        \end{center}
    \end{figure*}    

Algorithm~\ref{alg:Ccju} depicts how $C_{CJU}$ is calculated for a number of $n$-bit with $k$-bit block size. For example if block size $k = 6$, then the equation for $C_{CJU}$ will be equation~\ref{EQ6}.    
    \begin{equation}
        \label{EQ6}
         C_{CJU} = (A_5.B_5 + A_4.B_4 + A_3.B_3).P_0.P_1.ECT
    \end{equation}    
    
Line~\ref{line:8} of Algorithm~\ref{alg:Ccju} and equation~\ref{EQ6} shows that the expression for the propagation of carry from lesser significant bits has been considerably reduced (though the expression is prone to error). This leads to reduction in area , delay and power consumption which is discussed in detail in Section~\ref{sec:hard}. Hence we can conclude that,  %It can also be judged from the algorithm~\ref{alg:Ccju} and equation\ref{EQ6} that there will be no carry from lesser significant bits if $C_{CJU} = 0$. For example consider blocksize $k=6$ and a carry is generated by $5_{th}$ digit suppose this carry is killed by one of the most significant upper 3 bits then $C_{CJU} = 0$ which clearly implies that carry generated from lesser significant bits won't be able to get transmitted to next block.
there will be no carry generated from lesser significant bits if $C_{CJU} = 0$. For example, if we consider a block size $k=6$ and a carry is generated by $5^{th}$ bit. Suppose this carry is destroyed by one of the upper 3 bits, then $C_{CJU} = 0$.  
        %\item Above example clearly implies that carry generated from lesser significant bits won't be able to get transmitted to next block since $C_{CJU} = 0$.
        
The probability of error in computation of $C_{CJU}$ occurs when digits less significant than upper 3 bits destroys the carry generated by bits less significant than them. Since, probability for any bit to destroy a carry generated is $1/4$ ($A_i=0, B_i=0$), so our $C_{CJU}$ is correctly evaluated for considerable amount of cases of addition. Consider a block of size $k=6$ and carry is generated by $G_5$ as shown in equation~\ref{EQ3}. Suppose this carry generated is destroyed only by either ($A_4,B_4$) or ($A_3,B_3$). Then, removal of this error will not be detected by the terms in the expression for $C_{CJU}$ which could lead to a potential window for error. 

The probability of carry generated by $i^{th}$ bit ($i^{th}$ bit should be less significant than upper 3 bits) being correctly predicted by CJU depends on the equation~\ref{EQ7}. Since, carry generated is propagated $3/4$ (1-1, 0-1, 1-0 configuration) times by bits more significant than it. Hence, term $3/4$ is used in equation~\ref{EQ7} while the exponent $i-3$ in equation~\ref{EQ7} accounts for the CJU using only the carry propagation term of most significant upper 2 bits and an Error Correction Term (ECT) for $3^{rd}$ most significant bit. CJU  does not take into consideration the rest lesser significant propagation terms. Hence, lesser significant term bits need to propagate to predict the correct result.    
\begin{equation}
    P_{correct} = (3/4)^{i-3}
    \label{EQ7}
\end{equation}
An observation can also be made from the Algorithm~\ref{alg:Ccju}, equation~\ref{EQ6} and equation~\ref{EQ7} that as the distance of lesser significant bits decreases from the most significant upper 3 bits, the probability of carry propagation error of that bit also decreases. In conclusion, the CJU design of ACLA judges $C_{out}$ from the lesser significant bits intelligently while the ECU design of ACLA computes $C_{out}$ from the upper bits exactly. %Thus, justifying their name.           
        




==> Text/dummy.tex <==
\author{\IEEEauthorblockN{Michael Shell}
\IEEEauthorblockA{School of Electrical and\\Computer Engineering\\
Georgia Institute of Technology\\
Atlanta, Georgia 30332--0250\\
Email: http://www.michaelshell.org/contact.html}
\and
\IEEEauthorblockN{Homer Simpson}
\IEEEauthorblockA{Twentieth Century Fox\\
Springfield, USA\\
Email: homer@thesimpsons.com}
\and
\IEEEauthorblockN{James Kirk\\ and Montgomery Scott}
\IEEEauthorblockA{Starfleet Academy\\
San Francisco, California 96678--2391\\
Telephone: (800) 555--1212\\
Fax: (888) 555--1212}}

\begin{thebibliography}{1}

\bibitem{IEEEhowto:kopka}
H.~Kopka and P.~W. Daly, \emph{A Guide to \LaTeX}, 3rd~ed.\hskip 1em plus
  0.5em minus 0.4em\relax Harlow, England: Addison-Wesley, 1999.

\end{thebibliography}

==> Text/overhead.tex <==
\section{Overhead}
    \label{sec:overhead}

==> Text/related.tex <==
\section{Related Works}
    \label{sec:related}
Approximate adders and multipliers have served as the \textit{de-facto} building blocks for designing approximate systems. Towards this, there have been several approaches to designing innovative solutions for the same~\cite{nayar,alish}. %Bhattacharjya et al.~\cite{rajat} proposed a carry estimating technique for approximately adding two numbers, though their basic design CESA doesn't contain any multiplexer thereby saving area, however, their higher-accuracy variant CESA-PERL makes use of multiplexers so as to provide higher accuracy for larger computations which thereby results in higher on-chip area. 

Kanani et al.~\cite{alish} proposed an accuracy-configurable approximate adder based on carry-selection that can be configured for accuracy by varying the size of the carry chains. However, even in~\cite{alish}, they make use of multiplexers for their design which consumes higher on-chip area. RAP-CLA~\cite{rapcla} produces results that are 63.7\% more error-prone than an accurate adder. It also consumes more area and power as compared to CLA~\cite{cla}. 

In~\cite{nayar}, an approximate adder was proposed using root mean square error method. The architecture in~\cite{nayar} is divided into two-parts, namely, accurate and approximate parts. They also measured the performance of their adder using image processing application. %Approximate adders as shown in~\cite{eta,etai} break the input operands into two parts. Here, the most significant segment in computed accurately whereas the lesser significant segment is computed using approximate techniques.

%Mahdiani et al.~\cite{mahdi} proposed an approximate adder with two parts, namely, accurate and approximate. They called their design LOA. The lesser significant sum is computed using OR operations of corresponding lesser significant bits. However, the bit pair just before the more significant sum, in the lesser significant part is AND-ed so as to generate carry-in for the computation of the most significant part of the result.

In the designs proposed in~\cite{hu,kim}, the basic motivation is somewhat similar to the carry-select adder. Here, blocks are created and sum is calculated for individual blocks. The carry-in to respective blocks is either predicted to be 0 or 1 and the predicted carry is propagated rather than the actual carry.

In this paper, we investigate ACLA, an approximation mechanism proposed on the carry-lookahead adder. ACLA shows lesser area and power consumption as it does not employ any multiplexer in its design contrary to~\cite{sara,rapcla} and still provides very good accuracy compared to other state-of-the-art approximate adders. For power and area constrained environments such as embedded systems, ACLA serves as a suitable alternative to other state-of-the-art approximate adders as visible from section~\ref{sec:hard}. On application's end, ACLA produces results that are 23.57\% better than other state-of-the-art approximate adders.







==> Text/result.tex <==
\section{Results and Analysis}
    \label{sec:results}

In this section, we check the performance of ACLA with three applications.

    \subsection{Image Processing: Gaussian Smoothing}
    \begin{figure}[htbp]
            \begin{center}
                \includegraphics[width=0.48\textwidth]{Text/lena.png}
                
                \caption{Gaussian image smoothing (a) Original image, (b) Original image with noise, (c) RAP-CLA, PSNR=29.366dB \& SSIM=0.7814 (d) SARA, PSNR=26.79dB \& SSIM=0.787 (e) BCSA, PSNR=33.9dB \& SSIM=0.9142 (f) BCSA with ERU, PSNR=37.837dB \& SSIM=0.9482 (g) ACLA, PSNR=38.82 dB \& SSIM=0.9693}
                \vspace{-3.0ex}
                \label{fig:lena}
            \end{center}
        \end{figure}
        
    So as to measure the efficacy of ACLA, we performed Gaussian Smoothing on a 256x256 grayscale image of \textit{Lena}. We take a 5x5 floating-point kernel and round the values of it to fixed-point numbers as the approximate adders used perform fixed-point operations. The addition operation in convolution is approximated and the remainder of the math tasks are unaltered. 
    
    We compare ACLA's performance with respect to other state-of-the-art approximate adders based on Peak Signal to Noise Ratio (PSNR) and Structural Similarity Index (SSIM)~\cite{ssim}. The configuration of the approximate adders for this application are kept as, bit-size: 32-bit and block size: 8. The PSNRs and SSIMs of all the approximate adders are calculated with respect to accurate addition. Comprehensive evaluation shows that ACLA outperforms all other state-of-the-art approximate adders in this application as shown in Figure~\ref{fig:lena}. The results clearly show that ACLA has a PSNR of 38.82 dB which is 32.2\%, 45\%, 14.5\%, 2.6\% greater than RAP-CLA; SARA; BCSA and BCSA with ERU respectively. This makes ACLA a suitable choice for an adder in Gaussian Smoothing.
    
    \subsection{Trade-off analysis}
    
    \vspace{-2ex}
            \begin{figure}[h]
                \centering
                \includegraphics[width=0.35\textwidth]{Images/psnr.PNG}
		        \caption{PSNR vs ADP}
                \vspace{-0.ex}
		        \label{fig:psnr}
		        
            \end{figure}
    
    
    In Figure~\ref{fig:psnr}, an overall comparison between PSNR obtained from Gaussian Smoothing and overall hardware cost ADP (Area$\times$ Delay$\times$ Power) is shown. It is clearly visible that though the hardware cost of ACLA is more compared to RAP-CLA and SARA, ACLA shows significant benefit on PSNR over the other adders. On an average ACLA outperforms other state-of-the-art adders by 23.53\%. Hardware cost for ACLA is more compared to RAP-CLA because for bit size: 32 and block size: 8 (as (32, 8) configuration is kept for Gaussian Smoothing), according to equation~\ref{EQ6}, we have higher delay. The reason for higher hardware cost of ACLA in comparison with SARA is parallel use of two units ECU and CJU which leads to more power consumption. Significant delay is also there due to the implementation of a complex equation, i.e, equation~\ref{EQ6} specifically in the (32, 8) configuration. Compared to BCSA and BCSA with ERU, we can clearly see that ACLA wins by a significant margin by having a better PSNR and lower hardware cost. Hence, an overall view proves ACLA to be an efficient approximate adder for use in error-resilient applications. 
    
   So as to understand the trade-off between ADP and error parameters of ACLA, we need to understand that employment of an extra unit of CJU improves the delay-error statistics of the adder but compromises the area-power indicators. Similarly, using only upper 3 bits in ECU improves the ADP statistics but compromises the error indicators. Moreover, parallel computation by ECU and CJU enhance the delay indicators for the proposed approximate adder.      
%    \subsection{Analysis on Speedup}
%        Section~\ref{subsec:e_speedup} already explains the approach taken in order to study the speedup obtained by \shortx. On average, we obtain speedup of 2.28x and 3.59x for 32-bit, 8 block and 32-bit, 4 block configurations respectively. The results are self-explanatory as the amount of time spent on addition operations are reduced. Figure~\ref{fig:speedup} represents the aforementioned study. The \textit{base} adder used in this study corresponds to a conventional ripple-carry adder.
%        \begin{figure}[h]
%            \centering
%            \includegraphics[width=0.45\textwidth]{Images/speedup.pdf}
%            \caption{Analysis on Speedup}
%            \label{fig:speedup}
%        \end{figure}

    \subsection{Machine Learning Application}
        \subsubsection{K-Means}
            \label{subsubsec:kmeans}
            K-Means is a clustering algorithm used extensively in machine learning. The algorithm clusters a given set of data points into \textit{k} clusters. The similarity index used is usually euclidean distance metric. In this experiment, we have used a simple dataset containing roughly 150 points uniformly distributed into 3 clusters. At each iteration of the algorithm, the cluster centers are updated in order to find the best possible cluster. Since ACLA is an integer adder, we have quantized any floating point number, if encountered during computation, into its nearest integer.
            \begin{figure}[h]
                \centering
                \includegraphics[width=0.45\textwidth]{Images/acla-kmeans-f.pdf}
                \caption{Evaluation of K-Means using (a) accurate adder, (b) ACLA with (32, 8) configuration, and, (c) ACLA with (16, 8) configuration.}
                \label{fig:kmeans}
            \end{figure}    
            Figure~\ref{fig:kmeans} represents the outcome of the algorithm. Accurate clustering is depicted in Figure~\ref{fig:kmeans} (a). Out of every 3 trials in (32, 8) configuration ACLA incorrectly clusters one data point (Figure~\ref{fig:kmeans} (b)). Incorrectly clustered point in highlighted within a black box. The relative accuracy of the clustering algorithm in comparison with its accurate counterpart is 99.3\%. In (16, 8) configuration, represented by Figure~\ref{fig:kmeans} (c), up to 2 data points are incorrectly clustered, with relative accuracy falling to 98.6\%. The core principle of the algorithm, however, is lost when evaluated using all 8-bit configurations. 
        
        \subsubsection{kNN}
             kNN is a supervised classiﬁcation technique. For \shortx's evaluation, we have used two integer datasets including monk’s problem and Haberman’s survival~\cite{Dua:2019}. The principle behind kNN algorithm is to ﬁnd similarity between a given input set. The output is a class membership value of a given testing data point, which is assigned to its  k\textsuperscript{th} nearest neighbour. All the datasets are split into training and testing sets with a distribution ratio from 9:1 to 1:9 respectively. Comparison of classification is done using an accurate adder. For quantization of floating point numbers, a similar approach is taken as mentioned in Section~\ref{subsubsec:kmeans}. We have used Euclidean distance metric for similarity calculations. Final results are presented in terms of \textit{accuracy} and \textit{F1 score} of the dataset.
  
             The outcome of kNN is shown in Figure~\ref{fig:knn}, where Figure~\ref{fig:knn} (left) represents accuracy and F1 scores using an accurate adder. Our evaluation of ACLA shows no deviation in terms of both accuracy and F1 scores in configurations including (32, 8) and (16, 8). In the case of monk dataset, both accuracy and F1 scores were identical to an accurate adder in all 32-bit size and 16-bit size configurations. However, we see an absolute deviation of 1.12\% in terms of accuracy and 0.007 in terms of F1 scores for the Haberman's survival dataset when evaluated using (32, 4) configuration. \shortx's evaluation using (32, 4) bit size and block size configuration is depicted in Figure~\ref{fig:knn} (right).
             \vspace{-2ex}
            \begin{figure}[h]
                \centering
                \includegraphics[width=0.5\textwidth]{Images/knn_idx.PNG}
                \vspace{-8ex}
            \end{figure}              
            \begin{figure}[h]
                \centering
                \includegraphics[width=0.5\textwidth]{Images/knn-acla.pdf}
                \caption{Evaluation of kNN Algorithm using accurate adder (left), and, ACLA with (32, 4) configuration (right) on monk's problem and Haberman's survival dataset.}
                \vspace{-3ex}
                \label{fig:knn}
            \end{figure}  
